Tractable higher-order under-approximating AE extensions for non-linear systems

We consider the problem of under and over-approximating the image of general vector-valued functions over bounded sets, and apply the proposed solution to the estimation of reachable sets of uncertain non-linear discrete-time dynamical systems. Such a combination of under and over-approximations is very valuable for the verification of properties of embedded and cyber-physical controlled systems. Over-approximations prove properties correct, while under-approximations can be used for falsification. Coupled, they provide a measure of the conservatism of the analysis. This work introduces a general framework relying on computations of robust ranges of vector-valued functions. This framework allows us to extend for under-approximation many precision refinements that are classically used for over-approximations, such as affine approximations, Taylor models, quadrature formulae and preconditioning methods. We end by evaluating the efficiency and precision of our approach, focusing on the application to the analysis of discrete-time dynamical systems with inputs and disturbances, on different examples from the literature.

==> experiments.tex <==
%In Figures~\ref{fig2} and \ref{fig4}, the maximal under-approximation of the image (also called inner image), robust inner image, minimal inner image are respectively the dark blue, orange and red filled regions; the minimal over-approximation of the image (or outer image) is in blue and the maximal outer image in black lines. In Figure~\ref{fig2}, the "tentacles"  represent the vertices of the box over-approximations. %In Figure~\ref{fig3}, the caption is  explicit. 

We choose $\pi(i)=i$ for each state space-component $i$.
\subsection{Dubbins vehicle}

%- le outer joint range: en noir avec bcp de transparence
%	- le maximal inner : en bleu foncé 
%	- le robust inner : en orange
%	- le minimal inner : en rouge
%Ils sont affiches dans l’ordre ci-dessus, donc normalement si on ne voit que le minimal inner et pas le robust inner ca veut dire qu’ils sont egaux

We consider the classical Dubbins vehicle studied in \cite{decomposition-tomlin} with constant speed $v$ and angular control $a$, giving the dynamics of its position $(p_x,p_y)$ and its heading $\theta$. 
%The dynamical equations for a Dubins vehicle of constant speed $v$ are~: 
%$$\left(\begin{array}{c}
%\dot{p}_x \\
%\dot{p}_y \\
%\dot{\theta}
%\end{array}\right) = \left(\begin{array}{c}
%v cos(\theta)+b_1 \\
%v sin(\theta)+b_2 \\
%a+b_3
%\end{array}\right)
%$$
%\noindent where $a$ is the (angular) control, and $b=(b_1,b_2,b_3)$ is the disturbance. 
We set here $v = 5$, $a \in [-1,1]$, and disturbances $b_1, b_2, b_3$ to be added to each component of the dynamical system: $-1 \leq b_1 \leq 1$, $-1 \leq b_2 \leq 1$ and $-5 \leq b_3 \leq 5$. 

%In order to compare our method to other existing reachability methods, and for this example, to Hamilton-Jacobi-Bellman equation based methods, we compute outer and inner approximations of the
%backwards reachable set (BRS) of the system above. Recall that for a dynamical system of the form 
%$\dot{x}=f(x,u,v)$, where $u$ is the control of the system and $v$ is the (adversarial) disturbance signal, 
%the BRS at time $t$, for target set ${\cal G}_0$ is~:
%$${\cal G}(t)=\{x | \exists u, \forall v, \exists x_0 \in {\cal G}_0, x_0=\varphi^{f}(0 ; x,t,u,v))\}$$
%\noindent (with $\varphi^f(s;x,t,u,v)$ denoting the solution of O DE with vector field $f$ at time $s$, starting at time $t$ at state $x$, and with controls $u$ and disturbances $v$) or equivalently, 
%$${\cal G}(t)=\{x | \exists u, \forall v, \exists x_0 \in {\cal G}_0, x=\varphi^{-f}(t ; x_0,0,u,v))\}$$
%\noindent seen as a forward reachable set with the opposite vector flow\footnote{This is possible under suitable and classical assumptions on $f$ which hold on our example.}.
To compare with the HJB methods of \cite{decomposition-tomlin}, we compute the backward reachable set from 
target set at time $t$ ${\cal G}(t)=\{x_0 | \forall u_{\cal A}, \exists u_{\cal E}, \exists x \in {\cal G}_0, x=\varphi^{f}(t ; x_0,u))\}$ from the 
target set ${\cal G}_0=\{(p_x,p_y,\theta) | |p_x| \leq 0.5, |p_y|\leq 0.5, \ 0 \leq \theta \leq 2 \pi \}$. This is equivalent to computing  
$\{x_0 | \forall u_{\cal A}, \exists u_{\cal E}, \exists x \in {\cal G}_0, x_0=\varphi^{-f}(t ; x,u))\}$, the forward reachable set with the opposite vector flow.  
Figure \ref{pxpythetaDubbinsRINO} shows the robust  under-approximation, computed in 2 seconds,  
  with a Taylor method of order 3, a time horizon of 0.5 seconds and step size of 0.025 seconds, 50 subdivisions on the heading angle $\theta$, with constant controls and no disturbances. By subdividing an input, we mean here standard subdivision, leading to independent computations, to improve the precision of the approximation. We superpose  the corresponding under-approximations. The results are very similar to those shown in \cite{decomposition-tomlin}. Without disturbances, the maximal and robust reachable sets are equal.
%  The results, computed in 13.58 seconds  with a Taylor method of order 5, a time horizon of 0.5 seconds and step size of 0.01 seconds, 100 subdivisions on the heading angle $\theta$, with constant controls and no disturbances, are shown in Figure \ref{pxpythetaDubbinsRINO}. They are very similar to those shown in \cite{decomposition-tomlin}. 

%\ForAuthors{To be completed. Interpret and compare joint range ; time-varying controls ; disturbances}
% config_0_11_paper1.txt
\begin{figure}
%\begin{center}
%\begin{subfigure}{.225\linewidth}
%\epsfig{file=pxDubbinsRINO.png,clip=,width=4.5cm}
%\caption{$p_x$}
%\label{pxDubbinsRINO}
%\end{subfigure}
%\begin{subfigure}{.225\linewidth}
%\epsfig{file=pyDubbinsRINO.png,clip=,width=4.5cm}
%\caption{$p_y$}
%\label{pyDubbinsRINO}
%\end{subfigure}
%\begin{subfigure}{.225\linewidth}
%\epsfig{file=thetaDubbinsRINO.png,clip=,width=4.5cm}
%\caption{$\theta$}
%\label{thetaDubbinsRINO}
%\end{subfigure}
\begin{subfigure}{.48\linewidth}
\hspace{-.1cm}\epsfig{file=jointpxpythetaDubbins-new.png,clip=,width=4.5cm} % 7.5
\caption{With no disturbances}
\label{pxpythetaDubbinsRINO}
\end{subfigure}
%\caption{Dubbins vehicle, constant controls and no disturbances}
\begin{subfigure}{.45\linewidth}
\epsfig{file=jointpxpythetaDubbinsdisturb-new.png,clip=,width=4.9cm}
\caption{With disturbances}
\label{pxpythetaDubbinsRINOtimedisturb}
\end{subfigure}
%\caption{Dubbins vehicle, constant controls and no disturbances}
\caption{Joint $p_x$, $p_y$ and $\theta$ for Dubbins, constant controls}
\label{fig2}
%\end{center}
\end{figure}

Now we analyze the same system, but with disturbances, 
with the same parameters. The results, also obtained in 2 seconds, are shown in 
Figure \ref{pxpythetaDubbinsRINOtimedisturb}.  
The robust approximation, in orange, is now smaller, as expected. %, but still similar to the one computed in \cite{decomposition-tomlin}: i
Indeed, reaching the small centered unit square from any direction, under some disturbances, limits the potential initial positions, given the (controlled) angular speed's bounds. The maximal under-approximation, in light blue, is comparable to that of the unperturbed case.
%and with time-varying controls (piecewise-constant on a step size of 0.01 seconds), 
% JE n'arrive pas a avoir quelque chose d'interessant avec controles pas constants!
%still with 100 subdivisions on $\theta$. The results, obtained in 13.33 seconds, are shown in 
%Figure \ref{pxpythetaDubbinsRINOtimedisturb}. 
%The resulting robust approximation is much smaller, but still similar to the one computed in \cite{decomposition-tomlin}. % TO BE CHECKED
%, \ref{pyDubbinsRINOtimedisturb}, \ref{thetaDubbisRINOtimedisturb} and \ref{thetaDubbinsRINOtimedisturb}.
% config_0_11_paper2.txt

%\begin{figure}
%\begin{center}
%\begin{subfigure}{.225\linewidth}
%\epsfig{file=pxDubbinsRINO.png,clip=,width=4.5cm}
%\caption{$p_x$}
%\label{pxDubbinsRINO}
%\end{subfigure}
%\begin{subfigure}{.225\linewidth}
%\epsfig{file=pyDubbinsRINO.png,clip=,width=4.5cm}
%\caption{$p_y$}
%\label{pyDubbinsRINO}
%\end{subfigure}
%\begin{subfigure}{.225\linewidth}
%\epsfig{file=thetaDubbinsRINO.png,clip=,width=4.5cm}
%\caption{$\theta$}
%\label{thetaDubbinsRINO}
%\end{subfigure}
%%\end{figure}

% J'en suis la

%This seems reasonable, but I do not understand that e.g. $\theta$ seems to be between $0$ and
%$6$ whereas as $a$ is between $-1$ and $1$ and we start with $\theta=0$, we should get $\theta$ 
%at $t=0.5$ between $-0.5$ and $0.5$ as found out by RINO. 

 \subsection{10D hover quadrotor}

%\ForAuthors{Peut-etre dire un mot sur les "tentacles" pour repondre au referee CDC, si on a la place?}

We now consider the model of a hovering quadrotor described in \cite{decomposition-tomlin} and consisting of a 10-dimensional system
%$$\left(\begin{array}{c}
%\dot{p}_x \\
%\dot{v}_x \\
%\dot{\theta}_x \\
%\dot{\omega}_x \\
%\dot{p}_y \\
%\dot{v}_y \\
%\dot{\theta}_y \\
%\dot{\omega}_y \\
%\dot{p}_z \\
%\dot{v}_z
%\end{array}\right)=\left(\begin{array}{c}
%v_x+d_x \\
%g tan \theta_x \\
%-d_1 \theta_x + \omega_x \\
%-d_0\theta_x+n_0 S_x \\
%v_y+d_y \\
%g tan \theta_y \\
%-d_1 \theta_y+\omega_y \\
%-d_0 \theta_y + n_0 S_y \\
%v_z+d_z \\
%k_T T_z -g
%\end{array}\right)
%$$
%\noindent with $n_0=10$, $d_1=8$, $d_0=10$, $k_T=0.91$ %$m=1.3$ 
defining the 3D position $(p_x,p_y,p_z)$, the linear velocities $(v_x,v_y,v_z)$, the pitch and roll $(\theta_x,\theta_y)$, the pitch and roll rates $(\omega_x,\omega_y)$. 
%and $-\frac{\pi}{18} \leq S_x \leq \frac{\pi}{18}$, $-\frac{\pi}{18} \leq S_y \leq \frac{\pi}{18}$
%and $0 \leq T_z \leq 2g=19.62$. 
%Note that the effect of the disturbances being linear in a very simple manner, it is extremely easy to derive the (robust) BRS from the approximations we already have at hand (without having to solve yet the 3-quantifiers problem). 
%The variables are $(p_x,p_y,p_z)$ denoting the positions in the 3D space, $(v_x,v_y,v_z)$ the linear velocity, $(\theta_x,\theta_y)$ are the pitch and roll respectively, $(\omega_x,\omega_y)$ are the pitch and roll rates. 
The controls are $S_x$, $S_y$ in $[-\frac{\pi}{180},\frac{\pi}{180}]$ representing the desired pitch and roll angle, and $T_z \in [0, 19.62]$, the vertical thrust. Disturbances $(d_x,d_y,d_z)$ represent for instance the wind in the three axes. 
The target set is given as 
%\begin{align*}
%{\cal G}_0=\{(p_x,v_x,& \theta_x,\omega_x,p_y,v_y,\theta_y,\omega_y,p_z,v_z) | \\
$-1 \leq p_x, 
 p_y \leq 1$, $-2.5\leq p_z \leq 2.5$, 
$v_x=-1.5$, $\theta_x=0$, $\omega_x = 0$,  
$v_y=-1.8$, $\theta_y=0$, $\omega_y=0$, $v_z=1.2$.  
%\}
%\end{align*} 
%For the analysis, we restrict the controls to $-\frac{\pi}{180} \leq S_x \leq \frac{\pi}{180}$, $-\frac{\pi}{180} \leq S_y \leq \frac{\pi}{180}$ and $0 \leq T_z \leq 2g=19.62$. 
The results shown in 
Figure \ref{jointpxpypz10DRINO} %and %\ref{jointpxpy10DRINO}, 
%\ref{jointpypz10DRINO}, 
%\ref{thetax10DRINO}, and \ref{omegax10DRINO} 
are for the model without disturbances: they are computed  in 1.28 seconds for an order 4 Taylor method, a time horizon of 0.5 seconds with a step size of 0.01. 
% ./main 0 10 examples/config_0_10t_paper1.txt
The robust inner image in orange (the maximal range is equal here to the robust range and thus hidden as there is no disturbance) is very similar to the corresponding one in \cite{decomposition-tomlin}, without the need to consider a decomposition into smaller dimensional subsystems. Similar results are obtained for time-varying controls, but in 6.49 seconds.
% that, given the final velocities on $x$ and $y$ that are negative, we can only have come from upper right states in this picture. Similarly, as we wish to end up at an altitude between -2.5 and 2.5 with positive vertical velocity, we can come mostly from lower altitudes, except when a bit farther away in the $y$ coordinate (meaning more in the past), where, given the magnitude of the vertical thrust, it is possible that the quadrotor goes down after a while. 
%Figures \ref{thetax10DRINO} and \ref{omegax10DRINO} show the evolution, respectively, of the pitch and pitch rates that impact mostly the $x$ coordinates we may come from. 
%The figures show similar results as the one showed in \cite{decomposition-tomlin}, but there again, 
%For controls $S_x$, $S_y$ and $T_z$ that can vary every 0.01 seconds, the analysis gives very similar results in 6.49 seconds, %, see Figure \ref{jointpypz10DRINOtime} 
%except mainly for the pitch rate. %$\omega_x$, see Figures  \ref{omegax10DRINOtime} and \ref{jointpypz10DRINOtime}. 
%Indeed, we can reach much larger sets of angular velocities $\omega_x$ with non-constant controls, but we still reach essentially the same coordinates $p_y$ and $p_z$. 
%Now, let us consider 
In the disturbed model, where $d_x$, $d_y$ and $d_z$ are taken to be between -0.5 and 0.5 (analysis time of 1.22 seconds), we see in %. Computation takes 1.22 seconds and some of the results are shown in 
Figure 
%\ref{jointpxpy10DRINOdisturb}, 
\ref{jointpypz10DRINOdisturb} that the minimal under-approximation of the image in red is close to the robust and maximal under-approximations in orange and blue and maximal over-approximations in grey. It demonstrates both  that the analysis is very accurate and the hovering is very stable under the disturbances. %It demonstrates proves that the system is quite robust to disturbances. 
%\ref{thetax10DRINOdisturb}, and \ref{omegax10DRINOdisturb}. 
%As can be expected, the outer approximations are a bit bigger in presence of disturbances, 
%see e.g.
%Figure \ref{jointpxpy10DRINOdisturb}, 
%and the robust ranges show that we have still control of the 10D hover, even in the presence of these disturbances, see e.g. Figure \ref{jointpypz10DRINOdisturb}.

% ./main 0 10 examples/config_0_10ter_paper2.txt

%x3x7x10 thetax, thetay, vz
%x2x6x10 vx, vy, vz

%For the 3D slice on the left of Figure 9 from \cite{decomposition-tomlin} (reproduced above), we get, using %Flowstar, but with all disturbances $d_x$, $d_y$ and $d_z$ put to 0, the figures \ref{thetax10Dflowstar}, %\ref{px10Dflowstar} and \ref{py10Dflowstar} (the file that is used is in Appendix \ref{flowstarexperiments}, and with RINO, we find the results in figures \ref{thetax10DRINO},
%\ref{px10DRINO} and \ref{py10DRINO} (see the corresponding config file in Appendix \ref{RINOexperiments}). 

%\ForAuthors{No disturbances first, interpretation ; pictures not updated yet}

%\begin{figure}
%\begin{center}
%\begin{subfigure}{0.45\linewidth}
%\epsfig{file=thetax10DRINO.png,clip=,width=4.5cm,height=3.3cm}
%x3
%\caption{$\theta_x$ as a function of time}
%\label{thetax10DRINO}
%\end{subfigure}
%\begin{subfigure}{0.45\linewidth}
%\epsfig{file=omegax10DRINO.png,clip=,width=4.5cm,height=3.3cm}
%x4
%\caption{$\omega_x$ as a function of time}
%\label{omegax10DRINO}
%\end{subfigure}
%\caption{10D example, no disturbance, constant controls}
%\end{center}
%\end{figure}

\begin{figure}
\begin{center}
%\begin{subfigure}{0.3\linewidth}
%\epsfig{file=jointpxpy10DRINO.png,clip=,width=5.5cm}
%\caption{Joint range for $p_x$ and $p_y$}
%x1x5
%\label{jointpxpy10DRINO}
%\end{subfigure}
%\begin{subfigure}{0.225\linewidth}
%\epsfig{file=jointpypz10DRINO.png,clip=,width=4.5cm}
%x5x9
%\caption{Joint $p_y$ and $p_z$, no disturbance, constant controls}
%\label{jointpypz10DRINO}
%\end{subfigure}
%\begin{subfigure}{0.225\linewidth}
%\epsfig{file=jointpypz10DRINOtime.png,clip=,width=4.5cm}
%\caption{Joint $p_y$, $p_z$, no disturbance, time-varying controls}
% x5x9.png
%\label{jointpypz10DRINOtime}
%\end{subfigure}
\begin{subfigure}{0.45\linewidth}
\epsfig{file=jointpxpypz10DRINO.png,clip=,width=4.5cm}
%x5x9
\caption{Joint $p_x$, $p_y$ and $p_z$, no disturbance, constant controls}
\label{jointpxpypz10DRINO}
%x1x5x9
\end{subfigure}
\begin{subfigure}{0.45\linewidth}
\epsfig{file=jointpypz10DRINOdisturb.png,clip=,width=4.5cm}
\caption{Joint $p_y$ and $p_z$, disturbances, time-varying controls}
%x5x9
\label{jointpypz10DRINOdisturb}
\end{subfigure}
\caption{10D hovering example}
\label{fig4}
\end{center}
\end{figure}

% HOP J'en suis la ; il faut voir aussi les 3D
%x1x5x9 pour pxpypz

%\begin{figure}
%\begin{center}
%\begin{subfigure}{0.45\linewidth}
%\epsfig{file=omegax10DRINOtime.png,clip=,width=4.5cm,height=3.3cm}
%\caption{$\omega_x$ for hover 10D}
%\label{omegax10DRINOtime}
% x4_min_max
%\end{subfigure}
%\caption{10D example with time-varying controls}
%\end{center}
%\end{figure}


% disturb

%\begin{figure*}
%\begin{center}
%\begin{subfigure}{0.225\linewidth}
%\epsfig{file=thetax10DRINOdisturb.png,clip=,width=4.5cm,height=3.3cm}
%x3
%\caption{$\theta_x$}
%\label{thetax10DRINOdisturb}
%\end{subfigure}
%\begin{subfigure}{0.225\linewidth}
%\epsfig{file=omegax10DRINOdisturb.png,clip=,width=4.5cm,height=3.3cm}
%x4
%\caption{$\omega_x$}
%\label{omegax10DRINOdisturb}
%\end{subfigure}
%\begin{subfigure}{0.225\linewidth}
%\epsfig{file=jointpxpy10DRINOdisturb.png,clip=,width=4.5cm}
%x1x5
%\caption{Joint range for $p_x$ and $p_y$}
%\label{jointpxpy10DRINOdisturb}
%\end{subfigure}

%\begin{subfigure}{0.225\linewidth}
%\epsfig{file=jointpxpypz10DRINOdisturb.png,clip=,width=4.5cm,height=3.3cm}
%\caption{$\theta_x$}
%\label{thetax10DRINOdisturb}
%\end{subfigure}
%\caption{10D example with disturbances}
%\end{center}
%\end{figure*}

%\begin{figure}
%\begin{center}

%\end{center}
%\end{figure}


%\ForAuthors{Dire que l'on obtient des resultats comparables a Tomlin - sur 0.5 secondes cependant, et avec $S_x$ et $S_y$ dans un range moindre.}



% config_0_10ter-disturb.txt
 
%\ForAuthors{Also time-varying controls}

%The differences can probably be explained because we have no disturbance (which tend to shrink the reachable set - to be tried with the level set toolbox!). Also, the slices that are presented in Figure 9 of \cite{decomposition-tomlin} may well be the states for which the other 7 variables are sampled to the initial values $(v_x,v_y,\theta_x,\theta_y,\omega_x,\omega_y)=(-1.5,-1.8,1.2,0,0,0,0)$. 


